Credal Model Averaging for classification: representing prior ignorance and expert opinions

Bayesian model averaging (BMA) is the state of the art approach for overcoming model uncertainty. Yet, especially on small data sets, the results yielded by BMA might be sensitive to the prior over the models. Credal Model Averaging (CMA) addresses this problem by substituting the single prior over the models by a set of priors (credal set). Such approach solves the problem of how to choose the prior over the models and automates sensitivity analysis. We discuss various CMA algorithms for building an ensemble of logistic regressors characterized by different sets of covariates. We show how CMA can be appropriately tuned to the case in which one is prior-ignorant and to the case in which instead domain knowledge is available. CMA detects prior-dependent instances, namely instances in which a different class is more probable depending on the prior over the models. On such instances CMA suspends the judgment, returning multiple classes. We thoroughly compare different BMA and CMA variants on a real case study, predicting presence of Alpine marmot burrows in an Alpine valley. We find that BMA is almost a random guesser on the instances recognized as prior-dependent by CMA.

==> cma-bma-results.tex <==
\subsection{Results}
We let the size $n$ of the training set vary between 30 and 1500; beyond this value the amount of prior-dependent instances is negligible.
For each value of $n$ we perform 30 training - test experiments.
Some plots are truncated at $n$=600, since no further significant changes are observed going beyond 
this amount of data.
\hl{we call indeterminate.. \\}

\begin{figure}[!ht]
 \centering
\begin{subfigure}
 \centering
\begin{tikzpicture}[]
\begin{axis}[xlabel=$n$, ylabel=Accuracy, legend style={draw=none, legend pos=south east}, grid=major, xmin=0,xmax=600, height= 0.25 * \textheight, width= 0.45 * \textwidth,
every axis/.append style={font=\footnotesize},ymax=0.97,ymin=0.93]
\addplot[smooth,mark=*] table [col sep=comma, x=sample_size, y=Uniform_accuracy] {accuracy_utility.csv};
\addplot [smooth, thick, dashed,red,every mark/.append style={fill=red!80!black},mark=square*]
table [col sep=comma, x=sample_size, y=BB_accuracy] {accuracy_utility.csv};
\addplot [smooth,thick,mark=triangle]
table [col sep=comma, x=sample_size, y=Central_accuracy ] {accuracy_utility.csv};
\legend{IB prior, BB prior, NB prior}
\end{axis}
\end{tikzpicture}
\end{subfigure}

\begin{subfigure}
 \centering
\begin{tikzpicture}[]
\begin{axis}[xlabel=$n$, ylabel=AUC, legend style={draw=none, legend pos=south east}, grid=major, xmin=0,xmax=600, height= 0.25 * \textheight, width= 0.45 * \textwidth,
every axis/.append style={font=\footnotesize}]
\addplot[smooth,mark=*] table [col sep=comma, x=sample_size, y=Uniform_AUC] {accuracy_utility.csv};
\addplot [smooth, thick, dashed,red,every mark/.append style={fill=red!80!black},mark=square*]
table [col sep=comma, x=sample_size, y=BB_AUC] {accuracy_utility.csv};
\addplot [smooth,thick,mark=triangle]
table [col sep=comma, x=sample_size, y=Central_AUC] {accuracy_utility.csv};
\legend{IB prior, BB prior, NB prior}
\end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Accuracy and AUC of BMA under different priors.
The plots are truncated at
$n$=600 since after this value no further change is observed.}\label{fig:acc-bma}
\end{figure}

The most common indicator of performance for classifiers is the \textit{accuracy}, namely the proportion of instances correctly classified using 0.5 as probability threshold.
However, a skewed distribution of the classes can misleadingly inflate the value of accuracy. If for instance a species is absent from 90\% of the sites, a trivial classifier
which always returning absence would achieve 90\% accuracy without providing any information.
The AUC (area under the receiver-operating curve) \citep{fawcett2006introduction} is  a more robust measure of performance, not affected by the class unbalance.
AUC varies between 0.5 (random guessing) and 1 (perfect prediction).

Fig. \ref{fig:acc-bma} shows the mean accuracy and AUC of BMA using different priors over the models.
Both measures show an upward trend with $n$: larger training sets allow to better learn the model and
result in better predictions. The
impact of the prior over the models in both  accuracy and AUC is quite thin.
For sample sizes $n<100$, the IB prior seems slightly better than the others.
For larger sample sizes, there is no practical difference among the performance obtained using the different priors; it is well known 
that  the impact of the prior decreases with the size of the training set (the data overwhelm the prior).
Overall, BMA performs well on this data sets, as its accuracy is consistently superior to 93\% and its AUC is consistently superior to 0.8.






\begin{figure}[!htbp]
 \centering
 \includegraphics[width=7cm]{fig/marmot/compareCMAs/fracindet.pdf}
\caption{Fraction of prior-dependent instances for the different CMA variants.\label{fig:marm-indeterminate}}
\end{figure}

We now analyze the CMA results.
The  percentage of indeterminate classifications (\textit{indeterminacy}) is shown in Fig. \ref{fig:marm-indeterminate}.
The  indeterminacy consistently decreases with the sample size.
This is the well-known behavior of credal classifiers, which become more determinate
as more data are available.
NB-CMA$_{ign}$ generates the \textit{highest} number of indeterminate classifications;
IB-CMA$_{ign}$ generates the \textit{lowest} number of indeterminate classifications;
The reason of this behavior lies in the different definition of the credal sets and has been already discussed.
Interestingly,  prior knowledge allows NB-CMA$_{exp}$
to be way less indeterminate than  NB-CMA$_{ign}$.

CMA  divides the instances into two groups: the \textit{safe} and the \textit{prior-dependent} ones.
We therefore separately assess the accuracy  of BMA on the safe and on the prior-dependent instances.
If the CMA approach is effective, BMA should be much less reliable on the prior-dependent instances than on the safe ones.

\begin{figure}[!htb]
 \centering
\subfigure[IB-CMA vs BMA with IB prior.]{\includegraphics[width=7.5cm]{fig/marmot/detVSindet/CMAfix/marmot2ha_denpstar2bma_accuracy_boxplot.pdf}}
\subfigure[IB-CMA vs BMA with BB prior.]{\includegraphics[width=7.5cm]{fig/marmot/detVSindet/CMAfix/bb_marmot2ha_denpstar2bma_accuracy_boxplot.pdf}}
\subfigure[NB-CMA (ignorant) vs BMA with IB prior.]{\includegraphics[width=7.5cm]{fig/marmot/detVSindet/CMAignorant/marmot2ha_denpstar2bma_accuracy_boxplot.pdf}}
\subfigure[NB-CMA (expert) vs BMA with NB prior.]{\includegraphics[width=7.5cm]{fig/marmot/detVSindet/CMAexpert/CE_marmot2ha_denpstar2bma_accuracy_boxplot.pdf}}
\caption{The BMA accuracy sharply drops on the prior-dependent instances recognized by IB-CMA.
Each boxplot refers to 30 experiments.\label{fig:acc-free}}
\end{figure}

In the following we denote as IB-BMA, BB-BMA and NB-BMA the BMA learned using respectively
the IB prior ($\theta$=0.5), BB prior ($\alpha$=$\beta$=1) and NB prior.
Figure \label{fig:acc-free} (a) compares the accuracy
of IB-BMA on the instances recognized as safe and prior-dependent by IB-CMA.
The IB prior is included in the credal set of IB-CMA; thus when IB-CMA return the same class,
IB-BMA returns the same class. On the prior-dependent instances  the accuracy of BMA severely drops, getting almost close to random guessing. On a data set with two classes, random  guessing has accuracy=0.5; BMA achieves on average accuracy 0.6 on the prior-dependent instances,
only slightly better than random guessing. On the safe instances, the accuracy of BMA is well above 90\%.
CMA thus uncovers a small yet non-negligible set of instances over which BMA performs poorly because of prior-dependence.
The phenomenon is already known in the literature of the credal classification \citep{corani2008learning,corani2008credal}.
It has been moreover observed \citep{corani2008credal,2013:23:isipta} that on such instance the BMA posterior probabilities do not allow fully realizing that the classification is so unreliable.
The point is that BMA is learned under a single prior, and the obtained posterior
cannot account for sensitivy analysis.
To identify the prior-dependent instances without using CMA, one would need to cross-check the predictions of many BMAs, each induced with a different prior over the models.
This would be however very unpractical.

A substantial similar behavior is shown by the BB-BMA. Notice that the beta-binomial prior of BB-BMA is not included in the credal set of IB-CMA. In principle thus we cannot guarantee that
its classifications match those of IB-CMA when IB-CMA returns a single class.
Yet,  there are no big differences between the IB and the BB prior on this data set.
In particular the BB prior suffers a drop of accuracy very similar to that of the IB prior on the prior-dependent instances.


In Figure \label{fig:acc-free} (c) we compare the accuracy of IB-BMA on the instances recognized as safe and as prior-dependent by NB-CMA$_{ign}$.  The prior of IB-BMA is contained in the credal set of
NB-CMA$_{ign}$.
The situation is qualitatively similar to the previous  Figures \label{fig:acc-free} (a)--(b). Yet, the accuracy of BMA on the prior-independent instances is now higher; it is on average 70\%.
The point is that NB-CMA$_{ign}$ \textit{much} more indeterminate than IB-CMA.
The credal set of NB-CMA$_{ign}$ contains the credal set of IB-CMA. Thus, when
IB-CMA is indeterminate, so is NB-CMA; moreover, NB-CMA is indeterminate also on a further set of instances.
Since the average accuracy of IB-CMA does not change, necessarily the accuracy of IB-BMA is higher
when NB-CMA$_{ign}$ is indeterminate.

Eventually, we compare the accuracy of NB-BMA on the instances recognized as safe and as prior-dependent by NB-CMA$_{exp}$. Note that the prior of NB-BMA  is included in the credal set of NB-CMA$_{exp}$.
On average, the accuracy of NB-BMA on the prior-dependent instances is about 60\%. The situation is quite similar to the comparison of IB-BMA and IB-CMA.

\subsection{Utility measures}
\begin{figure}[!ht]
 \centering
\begin{subfigure}
 \centering
\begin{tikzpicture}[]
\begin{axis}[xlabel=$n$, ylabel=Accuracy/Utility, legend style={draw=none, legend pos=south east}, grid=major, xmin=0,xmax=600, every axis/.append style={font=\footnotesize}, height= 0.25 * \textheight, width= 0.45 * \textwidth,ymin=0.93,ymax=0.97]
\addplot[smooth,mark=*] table [col sep=comma, x=sample_size, y=Uniform_accuracy] {accuracy_utility.csv};
\addplot [smooth, thick, dashed,red,every mark/.append style={fill=red!80!black},mark=square*]
table [col sep=comma, x=sample_size, y=Fixed_util65] {accuracy_utility.csv};
\addplot [smooth,thick,mark=triangle]
table [col sep=comma, x=sample_size, y=Fixed_util80] {accuracy_utility.csv};
\legend{BMA (accuracy), IB-CMA ($u_{65}$), IB-CMA($u_{80}$)}
\end{axis}
\end{tikzpicture}
\end{subfigure}

\begin{subfigure}
 \centering
\begin{tikzpicture}[]
\begin{axis}[xlabel=$n$, ylabel=Utility ($u_{65}$), legend style={draw=none, legend pos=south east}, grid=major, xmin=0,xmax=600, 
every axis/.append style={font=\footnotesize}, height= 0.25 * \textheight, width= 0.45 * \textwidth,ymin=0.88,ymax=0.97]
\addplot[smooth,mark=*] table [col sep=comma, x=sample_size, y=Expert_util65] {accuracy_utility.csv};
\addplot [smooth, thick, dashed,red,every mark/.append style={fill=red!80!black},mark=square*]
table [col sep=comma, x=sample_size, y=Ignorance_util65] {accuracy_utility.csv};
\addplot [smooth,thick,mark=triangle]
table [col sep=comma, x=sample_size, y=Fixed_util65] {accuracy_utility.csv};
\legend{NB-CMA$_{\mbox{exp}}$, NB-CMA$_{\mbox{ign}}$, IB-CMA}
\end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}
 \centering
\begin{tikzpicture}[]
\begin{axis}[xlabel=$n$, ylabel=Utility ($u_{80}$), legend style={draw=none, legend pos=south east}, grid=major, xmin=0,xmax=600, 
every axis/.append style={font=\footnotesize}, height= 0.25 * \textheight, width= 0.45 * \textwidth,ymin=0.93,ymax=0.97]
\addplot[smooth,mark=*] table [col sep=comma, x=sample_size, y=Expert_util80] {accuracy_utility.csv};
\addplot [smooth, thick, dashed,red,every mark/.append style={fill=red!80!black},mark=square*]
table [col sep=comma, x=sample_size, y=Ignorance_util80] {accuracy_utility.csv};
\addplot [smooth,thick,mark=triangle]
table [col sep=comma, x=sample_size, y=Fixed_util80] {accuracy_utility.csv};
\legend{NB-CMA$_{\mbox{exp}}$, NB-CMA$_{\mbox{ign}}$, IB-CMA}
\end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Accuracies of IB-BMA versus utility of IB-CMA. The plot is truncated at
$n$=600 since after this value no further change of accuracies is observed.}\label{accu-util-ib-cma}
\end{figure}

To further compare the classifiers we adopt
the utility measures introduced in \cite{Zaffalon20121282}, which we briefly describe in the following.
The starting point is the \emph{discounted accuracy}, which  rewards a prediction containing $m$ classes with $1/m$ if it contains the true class and with 0 otherwise.
Within a betting framework based on fairly general assumptions, discounted-accuracy is the only score which satisfies some fundamental properties for assessing both determinate and indeterminate classifications.
In fact, for a determinate classification (a single class is returned)
discounted-accuracy corresponds to the traditional classification accuracy.
Yet discounted-accuracy has severe shortcomings.
Consider two medical doctors, doctor \textit{random} and doctor \textit{vacuous}, who should diagnose  whether a patient is \emph{healthy} or \emph{diseased}.  Doctor \textit{random} issues uniformly random diagnosis; doctor \textit{vacuous} instead always returns both
categories, thus admitting to be ignorant.  Let us assume that the hospital profits a quantity of money  proportional to the discounted-accuracy achieved by its doctors at each visit.  Both doctors have the same \textit{expected} discounted-accuracy for each visit,  namely $1/2$.  For the hospital, both doctors provide the same \textit{expected} profit from each visit, but with a substantial difference: the profit of doctor vacuous has no variance.  Any risk-averse hospital manager should thus prefer doctor vacuous over doctor random: under risk-aversion, the expected utility increases with expectation of the rewards  and decreases with their variance \citep{levy1979approximating}.
To model this fact, it is necessary to apply a utility function to the discounted-accuracy score assigned to each instance.
The utility function is designed as follows in \cite{Zaffalon20121282}: the utility of a correct and determinate classification (discounted-accuracy 1) is 1; the utility of a wrong classification (discounted-accuracy  0) is 0. Therefore, the utility of a traditional classifier corresponds to its accuracy.
The utility of an accurate but indeterminate classification consisting of two classes (discounted-accuracy 0.5)  is assumed to lie between 0.65 and 0.8. Two quadratic utility functions are derived, passing respectively  through $\{u(0)=0,u(0.5)=0.65,u(1)=1\}$ and  $\{u(0)=0,u(0.5)=0.8,u(1)=1\}$, denoted as $u_{65}$ and $u_{80}$ respectively.
Utility of credal classifiers and accuracy of determinate classifiers can be directly compared.
Interestingly, the $u_{65}$ and $u_{80}$ functions provides score which are numerically close 
to respectively the $F_1$ and $F_2$ metric, which have been used to score indeterminate classifications in \cite{jose2009learning}.

Figure \label{accu-util-ib-cma}(a) compares the accuracy of IB-BMA
with the utility of IB-BMA, considering both $u_{65}$ and $u_{80}$ as
utility functions.
In both cases the utility of IB-CMA is higher than the accuracy of IB-BMA;
the extension to imprecise probability is shown to be  valuable.
The gap is narrower under $u_{65}$  and larger under $u_{80}$, as the latter function
assigns higher value to the indeterminate classifications.
Moreover, the gap gets thinner as the sample size increases: as the data set grows large,
IB-CMA becomes less indeterminate and thus closer to IB-BMA.

In Figure \label{accu-util-ib-cma}(b) and (c)  we 
compare the different CMAs  using 
$u_{65}$ and $u_{80}$.
According to $u_{65}$, the best performing model is IB-CMA, followed
by NB-CMA$_{exp}$ and by NB-CMA$_{ign}$.
The function $u_{65}$ assign  a limited value to the indeterminate classifications.
Thus under this utility the most  determinate algorithm (IB-CMA) achieves the highest score;
the least determinate (IB-CMA$_{ign}$) achieves the lowest score.

The same situation is found under $u_{80}$, but only for small sample sizes ($n$ \textless 60).
For larger $n$,  IB-CMA$_{ign}$ becomes the highest scoring CMA.
The point is that  IB-CMA$_{ign}$ is the most imprecise model, and under $u_{80}$ the imprecision is highly rewarded.
Depending thus on the considered utility function, a different variant of CMA achieves the best performance.

This is fully reasonable: each CMA provides a different trade-off between informativeness and robustness. Moreover, the two utility function represents two quite different types of risk aversion.
Yet, it is somehow puzzling that IB-CMA$_{exp}$ is never ranked as the top CMA, despite being the only one which combines a flexible model of prior ignorance without a robust elicitation of prior knowledge.

A partial explanation is that  the utility measures are derived assuming all the errors to be equally costly.
Although they are possibly the most advanced score for credal classifiers,
such assumption is quite unrealistic for our case study, where missing a presence is likely to be much costlier than missing an absence.
It might be that the prior knowledge is therefore more useful at detecting presence
than at optimizing the 0-1 accuracy.
This is further confirmed by the fact that for instance no significant difference is observed
among the various BMAs in terms of accuracy or AUC; yet, 
the NB-BMA has consistently higher sensitivity (probability of predicting presence when the actual class is presence) than both IB-BMA and BB-BMA.
So far there are no score for credal classifier able to treat the cost-sensitive setup, and developing
them might be quite challenging.
It they will become available, it will be interesting scoring the various CMA allowing 
mislabeling a true presence is likely to be much higher than the cost of mislabeling an absence.
